At-Scale Sparse Deep Neural Network Inference with Efficient GPU Implementation

This paper presents GPU performance optimization and scaling results for inference models of the Sparse Deep Neural Network Challenge 2020. Demands for network quality have increased rapidly, pushing the size and thus the memory requirements of many neural networks beyond the capacity of available accelerators. Sparse deep neural networks (SpDNN) have shown promise for reining in the memory footprint of large neural networks. However, there is room for improvement in implementing SpDNN operations on GPUs. This work presents optimized sparse matrix multiplication kernels fused with the ReLU function. The optimized kernels reuse input feature maps from the shared memory and sparse weights from registers. For multi-GPU parallelism, our SpDNN implementation duplicates weights and statically partition the feature maps across GPUs. Results for the challenge benchmarks show that the proposed kernel design and multi-GPU parallelization achieve up to 180 tera-edges per second inference throughput. These results are up to 4.3x faster for a single GPU and an order of magnitude faster at full scale than those of the champion of the 2019 Sparse Deep Neural Network Graph Challenge for the same generation of NVIDIA V100 GPUs. Using the same implementation, we also show single-GPU throughput on NVIDIA A100 is 2.37$\times$ faster than V100.

==> 4_application.tex <==
\section{Multi-GPU Scaling}
\label{sec:multigpu}
In this section, we discuss our multi-GPU implementation of the optimized-fused kernel.
We use MPI to parallelize the sparse DNN inference across multiple GPUs on the Summit system
This work adopts a ``batch parallel'' strategy, where weights are replicated between GPUs and the features are partitioned evenly across GPUs.
As the inputs are propagated through the network, the number of non-zero features in each GPU's partition can become imbalanced.
Figure~\ref{fig:loadbalance} shows an example of this effect, with some GPUs receiving $2.49\times$ as many non-zeros as others.
This leads to poor scalability, which we correct with a simple load-balancing procedure outlined in Algorithm~\ref{alg:loadbalance}.
Figure~\ref{fig:loadbalance} also shows the corrected load-balance, and a communication matrix representing the volume of data moving between ranks during load-balancing.

\setlength{\textfloatsep}{8pt}% Remove \textfloatsep
\begin{algorithm}
  \caption{Outline of Load-Balancing Algorithm on CPU}
  \begin{algorithmic}[1]
    \STATE \texttt{MPI\_Allgather} communication for exchanging number of non-zero feature rows.
    \STATE  Re-partition non-zero rows to balance partitions.
    \STATE  Send and receive corresponding non-zero rows to new partitions.
    \STATE  Communicate global category indices of features accordingly.
    \STATE  Gather all category indices and sort them at Rank 0.
  \end{algorithmic}
  \label{alg:loadbalance}
\end{algorithm}

\begin{figure}[h]
    \centering
    \includegraphics[width=9cm]{Figures/load_balancing.pdf}
    \vspace{-2ex}
    \caption{Load balancing of features among 42 ranks and corresponding sparse communication map.}
    \label{fig:loadbalance}
\end{figure}


%\section{Application to Sparse DNN Inference}

%\subsection{Fusing ReLU and spMM Kernels}

%\subsection{MPI Parallelization}

%\subsection{Pruning Inactive Features}

%\subsection{MPI Load Balancing}

%\subsection{Adaptive spMM Kernel Selection}


%\section{Summary of Optimizations}

%\subsection{Kernel-Level Optimizations}
%\subsubsection*{ELL (Blocked) Zero-Padding}
%\subsubsection*{Register Tiling}
%\subsubsection*{Shared-Memory Tiling}
%\subsubsection*{Thread Coarsening}
%\subsubsection*{Half Precision}

%\subsection{Application-Level Optimizations}
%\subsubsection*{Fusing ReLU and spMM Kernels}
%\subsubsection*{Pruning Inactive Features}
%\subsubsection*{MPI Load Balancing}
%\subsubsection*{Adaptive spMM Kernel Selection}


==> 6_limitations.tex <==
\section{Limitations and Future Work}

==> 9_related.tex <==

\section{Related Work}

Argueta and Chiang ~\cite{argueta2019accelerating} describe a sparse matrix multiplication in the context of word embeddings, where a matrix $A$ comprising of one-hot or $N$-hot rows representing words from a corpus is multiplied by a dense matrix $B$ of word embeddings to create a dense product of embeddings just of the words represented by $A$.
This is a sparse $\times$ dense $=$ dense implementation, like we discuss in Section~\ref{}.
Their implementation assigns a single thread to each product value, without use of shared memory.
They observe speedups of $2$-$6\times$ on V100 and $0.25$-$4\times$ on Titan X over cuSPARSE.

\subsection{Comparison with Graph Challenge}

Wang, Lin, Yang, and Owens~\cite{wang2019accelerating} show an implementation that uses cuSparse to perform the inputs $\times$ weights operation, and a GPU-accelerated \texttt{Matrix::build} operation built from five kernels to create the ultimate sparse final CSR representation of the output features.
Like us, they observe that removing zeroed entries from the output features is essential for performance, and that load-balancing based on the structure of the input activations also has a large impacto n performance.


\subsection{Comparison with GPU SpGMM}

\subsubsection{2020}

``Sparse matrix partitioning for optimizing SpMV on CPU-GPU heterogeneous platforms''

\subsubsection{2019}

``Adaptive sparse matrix-matrix multiplication on the GPU''.

``Register-aware optimizations for parallel sparse matrix–matrix multiplication''

``Adaptive sparse tiling for sparse matrix multiplication''

``Optimization of GPU Kernels for Sparse Matrix Computations in Hypre''



``SpFlow: Memory-driven data flow optimization for sparse matrix-matrix multiplication''

``Accelerating Sparse Matrix Operations in Neural Networks on Graphics Processing Units''

``Generalized Sparse Matrix-Matrix Multiplication for Vector Engines and Graph Applications''

``Optimizing sparse tensor times matrix on GPUs''

``Performance evaluation and analysis of sparse matrix and graph kernels on heterogeneous processors''

``Adaptive Sparse Matrix-Vector Multiplication on CPU-GPU Heterogeneous Architecture''

\subsubsection{2018}

``Multithreaded sparse matrix-matrix multiplication for many-core and GPU architectures''.

``Register-based implementation of the sparse general matrix-matrix multiplication on gpus''

``Design principles for sparse matrix multiplication on the GPU''

``Memory-efficient sparse matrix-matrix multiplication by row merging on many-core architectures''

``High-performance sparse matrix-matrix products on Intel KNL and multicore architectures''

``Regularizing irregularity: bitmap-based and portable sparse matrix multiplication for graph data on GPUs''

``Optimizing Sparse Matrix-Matrix Multiplication for Graph Computations on GPUs and Multi-Core Systems''

\subsubsection{2017}
``High-performance and memory-saving sparse general matrix-matrix multiplication for nvidia pascal gpu''.

``Performance-portable sparse matrix-matrix multiplication for many-core architectures''



\subsubsection{2016}

``Exploiting multiple levels of parallelism in sparse matrix-matrix multiplication''

``On improving performance of sparse matrix-matrix multiplication on gpus''

``GPU-Accelerated Sparse Matrix-Matrix Multiplication for Linear Scaling Density Functional Theory''

``Balanced hashing and efficient gpu sparse general matrix-matrix multiplication''

\subsubsection{2015}
Section 2 of 
``Optimizing Sparse Matrix—Matrix Multiplication for the GPU''
Dalton, Olson, and Bell

``A framework for general sparse matrix--matrix multiplication on GPUs and heterogeneous processors''
Liu and Vinter

``GPU-accelerated sparse matrix-matrix multiplication by iterative row merging''.

``Fast sparse matrix multiplication on GPU''

``Fast sparse matrix and sparse vector multiplication algorithm on the GPU''

``Optimizing sparse matrix operations on gpus using merge path''

``Efficient sparse matrix multiplication on GPU for large social network analysis''

``LightSpMV: Faster CSR-based sparse matrix-vector multiplication on CUDA-enabled GPUs''

\subsubsection{2014}

``An efficient GPU general sparse matrix-matrix multiplication for irregular data''.

``Sparse matrix multiplication: The distributed block-compressed sparse row library''

``Fastspmm: An efficient library for sparse matrix matrix product on GPUs''


\subsubsection{2012}

``CUSP: Generic Parallel Algorithms for Sparse Matrix and GraphComputations''
Bell and Garland

``Parallel sparse matrix– matrix multiplication and indexing: Implementation and experiments''
Buluc and Gilbert

\subsubsection{???}

Nvidia cuSparse













\subsection{Comparison with Previous Sparse DNN Challenge Submissions}

Bisson and Fatica~\cite{bisson2019gpu}.

Davis, Aznaveh, and Kolodziej~\cite{davis2019write}

Ellis and Rajamanickam~\cite{ellis2019scalable}.

Wang et al~\cite{wang2019performance}

Mofrad, Melhem, Ahmad, and Hammoud~\cite{mofrad2019multithreaded}

Huang et al.~\cite{huang2019accelerating}
